Multiclass Yeast Segmentation in Microstructured Environments with Deep Learning

Cell segmentation is a major bottleneck in extracting quantitative single-cell information from microscopy data. The challenge is exasperated in the setting of microstructured environments. While deep learning approaches have proven useful for general cell segmentation tasks, existing segmentation tools for the yeast-microstructure setting rely on traditional machine learning approaches. Here we present convolutional neural networks trained for multiclass segmenting of individual yeast cells and discerning these from cell-similar microstructures. We give an overview of the datasets recorded for training, validating and testing the networks, as well as a typical use-case. We showcase the method's contribution to segmenting yeast in microstructured environments with a typical synthetic biology application in mind. The models achieve robust segmentation results, outperforming the previous state-of-the-art in both accuracy and speed. The combination of fast and accurate segmentation is not only beneficial for a posteriori data processing, it also makes online monitoring of thousands of trapped cells or closed-loop optimal experimental design feasible from an image processing perspective.

==> content/conferences_upcoming.tex <==
% !tex root= ../unet_main.tex
 
\clearpage
%\makebox[1\textwidth][c]{\huge{test}} \vspace{1cm}
\normalsize
\section*{Upcoming Conferences}

%\subsection{IEEE Conferences}
\begin{itemize}
	\item \textbf{IEEE CIBCB 2020}\hspace{1.2cm}$\bullet$$\bullet$
	\begin{itemize}
		\item \makebox[3.3cm][l]{submission deadline:} \textbf{03.07.2020}
		%\\ \makebox[3.3cm][l]{ } 15.07.2020 (late break abs.)
		\item \makebox[3.3cm][l]{format:} max. 8 page, less is ok%, (2 page late abs.)
		\item \makebox[3.3cm][l]{notification:} 07.08.2020
		\item \makebox[3.3cm][l]{camera ready:} 04.09.2020
		\item \makebox[3.3cm][l]{date:} 27-29.10.2020
		\item \makebox[3.3cm][l]{location:} fully virtual (Chile) 
		\item \makebox[3.3cm][l]{potential topics:} imaging, modelling, inference, (OED)
		\item IEEE International Conference on Computational Intelligence in Bioinformatics and Computational Biology
		\item \url{https://cibcb2020.uai.cl}
%		\item \makebox[3.3cm][l]{rank:} B3 (Qualis 2012) / C (ERA 2010)
	\end{itemize}\

	\item \textbf{IEEE BIBM 2020} \hspace{1.2cm}$\bullet$$\bullet$
	\begin{itemize}
		\item \makebox[3.3cm][l]{submission deadline:} \textbf{01.09.2020}
		\item \makebox[3.3cm][l]{format:} upto 8 pages (+other options)
		\item \makebox[3.3cm][l]{notification:} 30.10.2020
		\item \makebox[3.3cm][l]{camera ready:} 18.11.2020
		\item \makebox[3.3cm][l]{date:} 16-19.12.2020
		\item \makebox[3.3cm][l]{location:} $\rightarrow$ fully virtual
		\item \makebox[3.3cm][l]{potential topics:} bioinformatics
		\item IEEE International Conference on Bioinformatics and Biomedicine 
		\item \url{https://ieeebibm.org/BIBM2020/}
%		\item \makebox[3.3cm][l]{rank:} CCF B (best CCF conf.) B4 (Qualis 2012)
		\item \makebox[3.3cm][l]{acceptance:} $20\%$ over history of conf.
		\item lots of unets; classification and segmentation%		\item $10\%$ of papers segmentation; 
%		\item $20\%$ of papers classification
%		\item BIBM2016 acceptance: 70 regular papers and 81 short papers out of 366 submissions; claim 20\% regular, 20\% short acceptance; however there are 351 objects in the IEEE explorer for this conference
%IEEE BIBM \url{https://ieeebibm.org/BIBM2020/} submission: September 1, 2020 takes place in December 2020 in Korea  CCF rank B conference, B4 Qualis rank, highest ranking bio conference in CCF! \textbf{$20\%$ acceptance rate 2018 and 2016 (however thats for each regular and short papers)}, however, all 500 papers in the proceedings? roughly $1/10$ of papers seem to be on segmentation; $1/5$ papers are on classification; up to 8 page IEEE 2-column format\\
%BIBM2016\\-70 regular papers; 81 short papers; 366 submissions; claim 20\% regular, 20\% short acceptance; however there are 351 objects in the ieee explorer for this conference\\
	\end{itemize}\

	\item \textbf{IEEE MEMS 2021} \hspace{1.2cm}($\bullet$)
	\begin{itemize}
		\item \makebox[3.3cm][l]{submission deadline:} \textbf{10.09.2020}
		\item \makebox[3.3cm][l]{format:} 2 page abstract, 600 word
		\item \makebox[3.3cm][l]{date:} 24-28.01.2021
		\item \makebox[3.3cm][l]{location:} Munich, Germany	
		\item \makebox[3.3cm][l]{potential topics} $\mu$fluidics 
		\item Micro Electro Mechanical Systems
	(IEEE MEMS 2021)
		\item \url{https://www.mems21.org}
		\item acceptance rate around $40\%$, each poster oral 2009?
%		\item get co-operation with SH on something like this?
%		\item \makebox[3.3cm][l]{rank:} unranked - A? - better than EMBC?
	\end{itemize}\

\item \textbf{IEEE IECBES 2020}\hspace{1.2cm}($\bullet$)
	\begin{itemize}
		\item \makebox[3.3cm][l]{submission deadline:} \textbf{27.09.2020}
%		\item submission deadline: 27.09.2020 
		\item \makebox[3.3cm][l]{format:} 6 pages (4 pages in past)
		\item \makebox[3.3cm][l]{date:} 1-3.03.2021
		\item \makebox[3.3cm][l]{location:} Malaysia
		\item \makebox[3.3cm][l]{potential topics:} imaging; $\mu$fluidics
		\item IEEE EMBS Conference on Biomedical Engineering and Sciences
		\item \url{https://www.iecbes.org/#!}
		\item (HK recommended, seems to focus on human application)
	\end{itemize}\

-----------------------\ \ \ deadlines 2021\ \ \ -----------------------\\

	\item \textbf{IEEE EMBC 2021}\hspace{1.2cm}$\bullet$$\bullet$
	\begin{itemize}
		\item \makebox[3.3cm][l]{submission deadline:} \textbf{January 2021 (expected)}
		\item \makebox[3.3cm][l]{format:} 4 pages (2020)
		\item \makebox[3.3cm][l]{date:} 26-30.07.20201
		\item \makebox[3.3cm][l]{location:}  Guadalajara, Mexico		
		\item \makebox[3.3cm][l]{potential topics:} imaging; $\mu$-fluidics; synbio
		\item 43rd Conference of the IEEE Engineering in Medicine and Biology Society (EMBS)
		\item \url{https://embc.embs.org/2021/}
		\item premier IEEE EMBS conference
%		\item $75\%$ acceptance rate, premier IEEE EMBS conference, $\mu$fluidics, size sorting separation paper Chen2019
%		\item \makebox[3.3cm][l]{rank:} B1 (Qualis) / A (ERA)
	\end{itemize}\

	\item \textbf{IEEE CIBCB 2021} \hspace{1.2cm}%$\bullet$$\bullet$
	\begin{itemize}
		\item \makebox[3.3cm][l]{submission deadline:} \textbf{April 2021 (expected)}
		\item \makebox[3.3cm][l]{format:} max 8 page paper
		\item \makebox[3.3cm][l]{date:} October 2021
		\item \makebox[3.3cm][l]{location:} Melbourne
		\item \makebox[3.3cm][l]{potential topics:} imaging, modelling, inference, (OED)
		\item IEEE International Conference on Computational Intelligence in Bioinformatics and Computational Biology
		\item \url{https://cis.ieee.org/conferences/conference-calendar}
%		\item \makebox[3.3cm][l]{rank:} B3 (Qualis 2012) / C (ERA 2010)
	\end{itemize}\

	
	\item \textbf{$\mathbf{\mu}$TAS 2021}\hspace{1.2cm}$\bullet$$\bullet$
	\begin{itemize}
		\item \makebox[3.3cm][l]{submission deadline:}  \textbf{May/June 2021 (expected)}
		\item \makebox[3.3cm][l]{format:} 2 page abstract
		\item \makebox[3.3cm][l]{date:} October 2021 (expected)
		\item \makebox[3.3cm][l]{location:} Palm Springs, USA 
		\item \makebox[3.3cm][l]{potential topics:} $\mu$fluidics, '5.02 Single-Cell Analysis'
		\item Miniaturized Systems for Chemistry and Life Sciences
		($\mu$TAS 2020 CBMS)
		\item \url{https://microtas2021.org}
%		\item $60\%$ acceptance rate 2013, partially orals ($10\%$)
	\end{itemize}\



\item \textbf{IEEE BioCAS 2021} \hspace{1.2cm}($\bullet$)
	\begin{itemize}
		\item \makebox[3.3cm][l]{submission deadline:} June 2021 (expected)
		\item \makebox[3.3cm][l]{format:} 4 page
		\item \makebox[3.3cm][l]{date:} October 2021 
		\item \makebox[3.3cm][l]{location:} Berlin, Germany		
		\item \makebox[3.3cm][l]{potential topics:} imaging, $\mu$fluidics, OED
		\item IEEE  Biomedical Circuits and Systems Conference 
		\item \url{https://2020.ieee-biocas.org/sites/biocas20/files/documents/call-docs/biocas2020-cfp_web_09.pdf}
%		\item $55\%$-$70\%$ acceptance rate
	\end{itemize}\

\item \textbf{IEEE IECBES 2021}
\begin{itemize}
	\item \makebox[3.3cm][l]{submission deadline:} \textbf{August 2021} (expected)
	%		\item submission deadline: 27.09.2020 
	\item \makebox[3.3cm][l]{format:} 6 pages (4 pages in past)
	\item \makebox[3.3cm][l]{date:}  December 2021 (expected)
	\item \makebox[3.3cm][l]{location:} TBA
	\item \makebox[3.3cm][l]{potential topics:} imaging; $\mu$fluidics
	\item IEEE EMBS Conference on Biomedical Engineering and Sciences
	\item \url{https://www.iecbes.org/#!}
	\item (HK recommended, seems to focus on human application)
\end{itemize}\

	\item \textbf{IEEE BIBM 2021}\hspace{1.2cm}$\bullet$$\bullet$
\begin{itemize}
	\item \makebox[3.3cm][l]{submission deadline:} \textbf{August 2021} (expected)
	\item \makebox[3.3cm][l]{format:} upto 8 pages (+other options)
%	\item \makebox[3.3cm][l]{notification:} 30.10.2020
%	\item \makebox[3.3cm][l]{camera ready:} 18.11.2020
	\item \makebox[3.3cm][l]{date:} December 2021
	\item \makebox[3.3cm][l]{location:} Seoul, S. Korea	
	\item \makebox[3.3cm][l]{potential topics:} bioinformatics
	\item IEEE International Conference on Bioinformatics and Biomedicine 
	\item \url{https://ieeebibm.org/BIBM2020/}
%	\item \makebox[3.3cm][l]{rank:} CCF B (best CCF conf.)
	\item \makebox[3.3cm][l]{acceptance:} $20\%$ over history of conf.
	\item lots of unets; classification and segmentation

\end{itemize}\


%	\item \textbf{Conference}
%	\begin{itemize}
%		\item \makebox[3.3cm][l]{submission deadline:} DATE
%		\item \makebox[3.3cm][l]{format:} PAGES/ABSTRACT
%		\item \makebox[3.3cm][l]{date:} DATES
%		\item \makebox[3.3cm][l]{location:} LOCATION		
%		\item \makebox[3.3cm][l]{potential topics:} TOPICS
%		\item 
%		\item \url{}
%		\item NOTES
%	\end{itemize}\
-----------------------\ \ \ -------------------- \ \ \ -----------------------\\ %deadlines 2022
\newpage
%ADD measurement ones and WACV etc?!	
%
%\textbf{ISBI2021} 2021, April 13-16, in Nice France; {submission: Oct 15, 2020}; {Oz projects?} Ronnerberger presented overlapping instance segmentation paper here in 2018 ISBI ranked A (ERA)!
%
%ICPR second round submission is July 10\\ (first round finished) they even have previous bio work and 2D fluoro stuff; decent quality\ Final Decisions to Authors.
%September 30, 2020\\
%
%
%CCF ranks bio:\\
%A\\
%none\\
%
%B\\
%IEEE BIBM
%%IEEE BIBM \url{https://ieeebibm.org/BIBM2020/} submission: September 1, 2020 takes place in December 2020 in Korea  CCF rank B conference, B4 Qualis rank, highest ranking bio conference in CCF! \textbf{$20\%$ acceptance rate 2018 and 2016 (however thats for each regular and short papers)}, however, all 500 papers in the proceedings? roughly $1/10$ of papers seem to be on segmentation; $1/5$ papers are on classification; up to 8 page IEEE 2-column format\\
%%BIBM2016\\-70 regular papers; 81 short papers; 366 submissions; claim 20\% regular, 20\% short acceptance; however there are 351 objects in the ieee explorer for this conference\\
%
%ISMB \url{http://www.iscb.org/about-ismb} deadline passed for 2020 CCF rank B conference, 2nd highest ranking bio conference in CCF!\\
%
%RECOMB \url{} International Conference on Research in
%Computational Molecular Biology CCF rank B\\
%
%C\\
%APBC Asia Pacific Bioinformatics Conference\\
%ISBRA International Symposium on Bioinformatics Research and Applications\\ $35\%$ acceptance
%
%
%
%
%
%\clearpage
%	\item \textbf{Conference}
%	\begin{itemize}
%		\item \makebox[3.3cm][l]{submission deadline:} DATE
%		\item \makebox[3.3cm][l]{format:} PAGES/ABSTRACT
%		\item \makebox[3.3cm][l]{date:} DATES
%		\item \makebox[3.3cm][l]{location:} LOCATION		
%		\item \makebox[3.3cm][l]{potential topics:} TOPICS
%		\item 
%		\item \url{}
%		\item NOTES
%	\end{itemize}\
%	
%	\item \textbf{Conference}
%	\begin{itemize}
%		\item \makebox[3.3cm][l]{submission deadline:} DATE
%		\item \makebox[3.3cm][l]{format:} PAGES/ABSTRACT
%		\item \makebox[3.3cm][l]{date:} DATES
%		\item \makebox[3.3cm][l]{location:} LOCATION		\item \makebox[3.3cm][l]{potential topics:} TOPICS
%		\item FULL CONFERENCE NAME
%		\item \url{}
%		\item NOTES
%	\end{itemize}\
\end{itemize}


\newpage

